A Semantic Framework for PEGs

Parsing Expression Grammars (PEGs) are a recognition-based formalism which allows to describe the syntactical and the lexical elements of a language. The main difference between Context-Free Grammars (CFGs) and PEGs relies on the interpretation of the choice operator: while the CFGs' unordered choice e | e' is interpreted as the union of the languages recognized by e and e, the PEGs' prioritized choice e/e' discards e' if e succeeds. Such subtle, but important difference, changes the language recognized and yields more efficient parsing algorithms. This paper proposes a rewriting logic semantics for PEGs. We start with a rewrite theory giving meaning to the usual constructs in PEGs. Later, we show that cuts, a mechanism for controlling backtracks in PEGs, finds also a natural representation in our framework. We generalize such mechanism, allowing for both local and global cuts with a precise, unified and formal semantics. Hence, our work strives at better understanding and controlling backtracks in parsers for PEGs. The semantics we propose is executable and, besides being a parser with modest efficiency, it can be used as a playground to test different optimization ideas. More importantly, it is a mathematical tool that can be used for different analyses.

==> table-json.tex <==
% !TEX root = main.tex
\noindent{\tiny
\begin{tabular}{|p{0.065\textwidth}|p{0.04\textwidth}|p{0.04\textwidth}|p{0.03\textwidth}|p{0.03\textwidth}||p{0.03\textwidth}|p{0.035\textwidth}|p{0.03\textwidth}|}
\hline 
    \textbf{File (bytes)} &
\textbf{G}
 & 
\textbf{G+cut}
 & 
\textbf{\%}
 & 
\textbf{NB}
 & 
\textbf{G}
 & 
\textbf{G+cut}
&
\textbf{\%}
 \\
\hline 
 276 & 4.461 & 3.786 & 15.1\% & 2 & 2.078 & 2.122 & -2.1\%\\
\hline 
 872 & 8.569 & 7.589 & 11.4\% & 4.8 & 6.788 & 6.940 & -2.2\% \\
\hline 
 1k & 27.307 & 25.193 & 7.7\% & 5.6 & 8.564 & 8.678 & -1.3\%\\
\hline 
 2k & 28.252 & 26.143 & 7.5\% & 5.4 & 12.736& 12.906& -1.3\%\\
\hline 
 4k & 31241 & 29.562 & 5.4\% & 4.8 & 23.101 & 23.417& -1.3\%\\
\hline 
 4k & 64.365 & 62.298 & 3.2\% & 6.4 & 24.395 & 24.696 & -1.2\%\\
\hline 
 6k & 114.596 & 113.812 & 0.7\% & 5.8 & 40.222 & 40.811& -1.4\%\\
\hline 
 10k & 102.401 & 101.365 & 1.0\% & 5 & 63.169 & 63999 & -1.3\%\\
\hline 
 14k & 120.876 & 119.714 & 1.0\% & 6 & 90.058 & 91.196 & -1.2\%\\
 \hline
\end{tabular}
}

